Towards Pragmatic Production Strategies for Natural Language Generation Tasks

This position paper proposes a conceptual framework for the design of Natural Language Generation (NLG) systems that follow efficient and effective production strategies in order to achieve complex communicative goals. In this general framework, efficiency is characterised as the parsimonious regulation of production and comprehension costs while effectiveness is measured with respect to task-oriented and contextually grounded communicative goals. We provide concrete suggestions for the estimation of goals, costs, and utility via modern statistical methods, demonstrating applications of our framework to the classic pragmatic task of visually grounded referential games and to abstractive text summarisation, two popular generation tasks with real-world applications. In sum, we advocate for the development of NLG systems that learn to make pragmatic production decisions from experience, by reasoning about goals, costs, and utility in a human-like way.

==> sections/modelling.tex <==
% ====================================
\section{Modelling}
\label{sec:modelling}
% ====================================

The Rational Speech Act framework offers the tools to include all these communicative costs. A pragmatic speaker $S'$ will produce an utterance according to the utility of that utterance given the intended future state of the world $w$ and the established linguistic context of the interaction $c$:
\begin{align}
    P_{S'}(u|w,c) \propto \exp \left( \alpha U_{S'}(u,w,c) \right)
    \label{eq:ps_u_wl}
\end{align}
The utility of a rational pragmatic speaker is typically defined recursively in terms of utterance cost and the (negative) surprisal of a pragmatic listener $L'$:
\begin{align}
    U_{S'}\left(u,w,c\right) = \log P_{L'}\left(w|u,c \right) - cost_S\left( u,c \right)
    \label{eq:us_uwl}
\end{align}
As previously discussed, the utterance production cost can be defined in multiple ways. All of the following definitions are with respect to a literal speaker $S$ that is unaware of the communicative goal; this is done to separate the purely linguistic constraints from the situational ones.
\begin{align}
    cost_S\left( u,c \right) = f(|u|)
    \label{eq:costs_u_len}
\end{align}
\begin{align}
    cost\left( u,c \right) = g(depth(u))
    \label{eq:costs_u_depth}
\end{align}
\begin{align}
    cost\left( u,c \right) = - \log P_S\left(u|c \right)
    \label{eq:costs_u_lm}
\end{align}
The interpretation of a pragmatic listener depends on the utility of that interpretation:
\begin{align}
    P_{L'}\left(w|u,c \right) \propto \exp\left(\beta U_{L'}\left(w,u,c \right) \right)
    \label{eq:costs_u_lm}
\end{align}
where the listener's utility is directly connected to the communicative goal and modulated by the processing effort of a literal listener:
\begin{align}
    U_{L'}\left(w,u,c \right) = R\left(w\right) + \log P_L\left(u|w,c\right)
    \label{eq:costs_u_lm}
\end{align}
The reward $R\left(w,u,c\right)$ depends on whether the communicative goal is achieved. I.e., it depends on whether the new state of the world $w$ is the one intended by the speaker. In a reference game, for example, the reward can be defined as follows:
\begin{align}
    R\left(w \right) = \begin{cases}
    1,& \text{if } w=w^{*}\\
    0,              & \text{otherwise}
\end{cases}
\end{align}
or:
\begin{align}
    R\left(w \right) = \log P_L(w|u,c)
\end{align}
where $w^{*}$ is the image targeted by the speaker's utterance.

\subsection{Recap}
Expanding Eq. 1 using Eq. 2,5,6,7,9 we can see that there are three important quantities that regulate the lexical choices of a speaker:
\begin{align}
    - \log P_S\left(u|c \right)\\
    - \log P_L\left(u|w,c \right)\\
    - \log P_{L}\left(w|u,c \right)
\end{align}
These are the production, processing, and comprehension effort, respectively.

